Anonymity Properties of the Bitcoin P2P Network

Bitcoin is a popular alternative to fiat money, widely used for its perceived anonymity properties. However, recent attacks on Bitcoin's peer-to-peer (P2P) network demonstrated that its gossip-based flooding protocols, which are used to ensure global network consistency, may enable user deanonymization---the linkage of a user's IP address with her pseudonym in the Bitcoin network. In 2015, the Bitcoin community responded to these attacks by changing the network's flooding mechanism to a different protocol, known as diffusion. However, no systematic justification was provided for the change, and it is unclear if diffusion actually improves the system's anonymity. In this paper, we model the Bitcoin networking stack and analyze its anonymity properties, both pre- and post-2015. In doing so, we consider new adversarial models and spreading mechanisms that have not been previously studied in the source-finding literature. We theoretically prove that Bitcoin's networking protocols (both pre- and post-2015) offer poor anonymity properties on networks with a regular-tree topology. We validate this claim in simulation on a 2015 snapshot of the real Bitcoin P2P network topology.

==> intro-complete.tex <==
\section{Introduction}
Cryptocurrencies are digital currencies in which transactions are verified cryptographically. 
They have surged in popularity over the last decade, with Bitcoin \cite{bitcoin} (the most common cryptocurrency) recently reaching a market capitalization of nearly \$20 billion \cite{btcmarket}.
Spurred in part by popular media, many users turn to Bitcoin as a privacy-preserving financial alternative to standard banking systems \cite{bitcoinprivacy,coinbase}.
However, Bitcoin was never designed for privacy.
Its primary goal is \emph{transparency}: users should be able to verify network transactions in a decentralized fashion. 
In service of this goal, Bitcoin users are assigned (possibly time-varying) pseudonyms, which do not inherently provide anonymity.
Indeed, the original Bitcoin paper explicitly states that in order to maintain any privacy, user pseudonyms should remain unlinkable to the user's true identity \cite{bitcoin}. 

In practice, there are several ways to deanonymize a user.
The most commonly-studied methods link Bitcoin pseudonyms to users' true identities by analyzing transaction patterns \cite{ober2013structure,reid2013analysis}. 
In this paper, we are interested in a lower-layer vulnerability: the networking stack.
Like most cryptocurrencies, Bitcoin nodes communicate over a P2P network \cite{bitcoin}. 
The anonymity implications of this P2P network have been largely ignored until recently, when several papers demonstrated empirical anonymity attacks on it \cite{biryukov,koshy2014analysis}. 
In this work, we study Bitcoin's networking protocols through a theoretical lens, and analyze their anonymity properties. 
Critically, we find that Bitcoin's anonymity properties are even worse than the practical attacks in \cite{biryukov,koshy2014analysis} suggested.
To more clearly state the problem, we begin with a brief introduction to Bitcoin.


\subsection{Bitcoin and Its P2P Network}
Bitcoin represents each user and each unit of Bitcoin currency by a public-private key pair.
A user ``possesses'' a coin by knowing its private key.
Any time a user Alice wishes to transfer her coin $m$ to Bob, she generates a signed \emph{transaction} message, which states that Alice (denoted by her public key) transmits $m$ (denoted by its public key) to Bob (denoted by his public key).
This transaction message is broadcast to all active Bitcoin nodes, at which point \emph{miners}, or nodes who volunteer to validate transactions, race to append the transaction to a global ledger known as the \emph{blockchain}.
Specifically, each miner aggregates a group of transaction messages into a \emph{block}, or list, and then completes a computational proof-of-work for the block;
the first miner to complete a proof-of-work appends their block to the blockchain and reaps a reward of newly-minted bitcoins and transaction fees.

%\subsubsection{Broadcasting Transactions}
This paper focuses on one key aspect of the above pipeline:  broadcasting transactions to other nodes.
The broadcasting process is critical because it affects which nodes can reap a transaction's mining reward: 
if a node receives a transaction late, its chances of reaping the mining reward for that transaction are reduced.
The broadcasting process also affects the network's global consistency: 
if only a subset of users receive a given transaction, then the transaction originator (i.e., the individual who spent the coin) can double-spend her coins.

To understand the mechanics of broadcasting, note that cryptocurrencies can be abstracted into two layers: the application layer and the network layer.
The application layer handles tasks like transaction management, blockchain processing, and mining.
In the application layer, nodes are identified by their public keys, which act as pseudonyms.
The network layer handles communication between nodes, which occurs over a P2P network of  TCP connections.
In the network layer, nodes are identified by their IP addresses.
As we shall see momentarily, a node's IP address and public key should remain unlinkable for privacy reasons.
%The P2P network is formed by having each node establish up to eight TCP connections with other nodes. %, whose IP addresses are stored either in a global DNS server or in users' local address books.

Bitcoin's peer-to-peer broadcast of transactions and blocks is based on flooding
information along links in the P2P network.
The protocols for flooding content have been the subject of some discussion, and are central to our paper. %; we  present  relevant flooding protocols in Section \ref{sec:model}.
In particular, we are interested in understanding the anonymity properties of existing flooding protocols.
%When a node learns of a new transaction or block, it floods the message to
%its neighbors who have not yet seen the message.
%%Neighbors who do not yet have the message request it, and receive the full message.
%%an \texttt{INV} message containing
%%the item's hash to each of its neighbors.
%%In response, if a given neighbor does not yet have that item, it requests
%%it with a \texttt{GETDATA} message. The original peer responds
%%with a \texttt{TX} or \texttt{BLOCK} message containing the relevant data.
%%Finally, because those neighbors have learned about a
%%new transaction or block, the
%The process continues recursively
%until all reachable peers receive the message.
%This broadcast forms the basis
%of Bitcoin's global, eventually consistent log, and is
%therefore of utmost importance to its correct and fair operation.

\vspace{0.1in}
\noindent \textbf{Anonymity in the Bitcoin  P2P network.}
%%\anote{what are the properties we require, and why is this so important? A) forking attacks and double spends, B) economic consequences of unreliable service, C) aligned incentives}
%Bitcoin's network layer should exhibit two principal properties: low latency and anonymity.
%
%\noindent \textbf{Low latency} means that the maximum time for a message to reach all network nodes should be bounded and small.
%Latency matters because if the network fails to deliver messages within a predictable time bound, the network risks reaching an inconsistent state.
Although Bitcoin was not designed to provide anonymity, it is nonetheless a critical property: an adversary should be unable to link transaction messages (and hence, the associated public keys) to the IP address that originated a transaction.
Recall that every transaction made by a public key is listed in plaintext in the blockchain.
Therefore, if a public key can be linked to an IP address, the adversary can link all of that user's transactions.
In some cases, the IP address could even be used to learn a node operator's human identity.
Thus, deanonymization attacks could result in a user's entire banking history being revealed.
%Cryptocurrency users are often recommended to choose fresh public keys and ``mix'' their coins to obscure their transaction histories~\cite{coinshuffle,mixcoin}, but in practice, few users do so~\cite{coinseer,fistful}. 
%Moreover, these techniques are useless if the IP address of the source of the transaction can be recovered.

In recent years, security researchers demonstrated multiple deanonymization attacks on the Bitcoin P2P network.
These attacks typically use a ``supernode" that connects to active Bitcoin nodes and listens to the transaction traffic relayed by honest nodes \cite{koshy2014analysis,biryukov,biryukov2015bitcoin}.
Using this technique, researchers were able to link Bitcoin users' public keys to their IP addresses with an accuracy of up to 30\% \cite{biryukov}.
%The source estimators used in these papers are simple, and exploit only minimal knowledge of the P2P graph structure and broadcasting protocols.
%We hypothesize that  higher accuracies may be possible with more sophisticated estimation tools.

In 2015, the Bitcoin community responded to these attacks by changing its broadcasting protocols from a gossip-style flooding protocol known as \emph{trickle spreading} to a \emph{diffusion spreading} protocol that spreads content with independent exponential delays \cite{bitcoindTrickleDiffusion}. 
We define these protocols precisely in Section \ref{sec:model}.
However, no systematic motivation was provided for this change. 
Indeed, it is unclear whether the change actually defends against the deanonymization attacks in \cite{biryukov,koshy2014analysis}. 

This problem is significant in part because Bitcoin's networking codebase is copied almost directly in other cryptocurrencies, or altcoins.
Anonymity vulnerabilities in Bitcoin's network therefore extend to a host of other altcoins.
Moreover, the research community has largely ignored the anonymity properties of the Bitcoin networking stack until recently, and there have been no efforts (to the best of our knowledge) to systematically analyze them. 
%Moreover, 
%To some extent, this is to be expected:
%Bitcoin's networking stack was taken directly from Satoshi Nakamoto's original network implementation, which  appears to have been a product of expediency.
%However, in the decade since Bitcoin's release,  the networking stack and its  anonymity properties have been largely ignored.
%%Our goal is to redesign it with anonymity in mind.



\subsection{Problem and Contributions}
Our goal is to analyze the anonymity properties of the Bitcoin P2P network.
The main point of our paper is to show that the Bitcoin network has poor anonymity properties, 
and the community's shift from trickle spreading (pre-2015) to diffusion spreading (post-2015) did not help the situation. 
Note that the optimal (maximum-likelihood) source-identification algorithms may change between protocols;
identifying such algorithms and quantifying their performance is the primary focus of this work.
We find that trickle and diffusion exhibit roughly the same poor anonymity properties.
Specifically, our contributions are threefold:



\vspace{0.07in}
\noindent \textbf{(1) Modeling.} We model the Bitcoin P2P network and an `eavesdropper adversary', whose capabilities reflect recent practical attacks in \cite{biryukov,koshy2014analysis}. 
This task is complicated by the fact that most Bitcoin network protocols are not explicitly documented. 
Modeling the system therefore requires parsing a combination of documentation, papers, and code. 
Several of the resulting models are new to the rumor source analysis literature.

\vspace{0.07in}
\noindent \textbf{(2) Analysis of Trickle (Pre-2015).} We analyze the probability of deanonymization by an eavesdropper adversary under trickle propagation, which was used until 2015. 
Our analysis is conducted over a regular tree-structured network.
Although the Bitcoin network topology is not a regular tree, we will see in Section \ref{sec:model} that regular trees are a reasonable first-order model.
We consider suboptimal, graph-independent estimators (e.g., the first-timestamp estimator), as well as maximum-likelihood estimators; both are defined precisely in Section \ref{sec:model}. 
Our analysis suggests that although the first-timestamp estimator performs poorly on high-degree trees, maximum-likelihood estimators can achieve high probabilities of detection for trees of any degree $d$ (Table \ref{tab:results}).


\vspace{0.07in}
\noindent \textbf{(3) Analysis of Diffusion (Post-2015).} 
We conduct a similar analysis of diffusion spreading, which was adopted in 2015 as a fix for the anonymity weaknesses observed under trickle propagation \cite{biryukov,koshy2014analysis}. 
Table \ref{tab:results} summarizes a subset of our results, which characterize the probability of detection  asymptotically in tree degree $d$. % diffusion performs similarly to trickle propagation. %, as seen in Table \ref{tab:results}. 
We wish to highlight the fact that trickle and diffusion exhibit similar anonymity behavior.
%The exact expressions in this table are less important than the fact that trickle and diffusion have similar behavior.
We revisit this table  more carefully in Section \ref{sec:experiments}, where we also empirically validate our findings on a snapshot of the real Bitcoin network from 2015. 
%Simulations confirm our theoretical results suggesting that diffusion does not significantly improve anonymity compared to trickle spreading.  

\begin{table}[t]
\centering
\caption{Summary of  probability of detection results on regular trees. Asymptotics are in the tree degree $d$. Notice that results for trickle and diffusion are similar. }% in the 2nd and 3rd rows.}
\label{tab:results}
\begin{tabular}{|c|c|c|}
\hline
                                                           & \begin{tabular}[c]{@{}c@{}}{\bf Trickle} \\ {\bf (pre-2015)} \end{tabular}&\begin{tabular}[c]{@{}c@{}} {\bf Diffusion} \\ {\bf (post-2015)}\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}{\bf First-}\\ {\bf Timestamp}\end{tabular} &    \begin{tabular}{@{}c@{}} $\frac{\log(d)}{d \log(2)} + o\left( \frac{\log d}{d}\right)$ \\ (Eq. \ref{eq:trickle1d})  \end{tabular}  &     \begin{tabular}{@{}c@{}} $\frac{\log(d-1)}{(d-2)}$ \\ (Thm. \ref{thm:fs_diffusion})     \end{tabular}   \\ \hline
\begin{tabular}[c]{@{}c@{}}{\bf Maximum-}\\ {\bf Likelihood}\end{tabular}                                                 &  $\Theta (1)$ ~ (Thm. \ref{thm:ml_trickle})        &     $\Theta (1)$ ~ (Thm \ref{thm:rc_diffusion})       \\ \hline
\end{tabular}
%\begin{tabular}{|c|c|c|c|}
%\hline
%\multicolumn{2}{|l|}{}                     & {\bf Trickle} & {\bf Diffusion} \\ \hline
%\multirow{2}{*}{\begin{tabular}{@{}c@{}} {\bf First-} \\ {\bf Timestamp} \end{tabular}} & All $\theta$ &   $ \frac{\theta}{\log 2} \left[\text{Ei}(2^d \log \rho) -\text{Ei}\left ( \log \rho \right ) \right ]$  ~ (Thm \ref{thm:fs_trickle})   &  $\frac{\theta d}{d-1}\log \frac{d(1+\theta) - 1}{\theta d}$ ~ (Thm. \ref{thm:fs_diffusion})      \\ \cline{2-4} 
%                           & $ \tiny{\theta = \frac{1}{d}} $    &  $\frac{\log(d)}{d \log(2)} + o\left( \frac{\log d}{d}\right)$ ~ (Eq. \ref{eq:trickle1d})        &    
%                           		$\frac{\log(d+1)}{d}$ ~ (Thm. \ref{thm:fs_diffusion})      \\ \hline
%{\bf Centrality}                 &               &   $\Theta (1)$ ~ (Thm. \ref{thm:ml_trickle})       &     $\Theta (1)$ ~ (Thm \ref{thm:rc_diffusion})       \\ \hline
%\end{tabular}
\end{table}

\vspace{0.1in}
\noindent \textbf{Paper Structure.}
We begin by modeling Bitcoin's P2P networking stack and the adversaries of interest in Section \ref{sec:model}.
We then analyze the performance of trickle propagation in Section \ref{sec:trickle}.
In Section \ref{sec:diffusion}, we analyze the performance of diffusion.
We compare these results side-by-side in Section \ref{sec:experiments}, which also includes empirical trials on a snapshot of the real Bitcoin network.
We discuss the relation between our results and prior work in Section \ref{sec:related}.
Section \ref{sec:discussion} concludes by discussing the practical implications of these results and preliminary ideas on how to solve the problem. 



